Inceptive Event Time-Surfaces for Object Classification Using Neuromorphic Cameras

This paper presents a novel fusion of low-level approaches for dimensionality reduction into an effective approach for high-level objects in neuromorphic camera data called Inceptive Event Time-Surfaces (IETS). IETSs overcome several limitations of conventional time-surfaces by increasing robustness to noise, promoting spatial consistency, and improving the temporal localization of (moving) edges. Combining IETS with transfer learning improves state-of-the-art performance on the challenging problem of object classification utilizing event camera data.

==> backup.tex <==
\iffalse
Inceptive Event Time Surfaces attempt to improve object classification success of HATS by creating RGB images from each data sample. The RGB image is generated from a statistical combination of the events. Instead of mapping pixels into cells, IETS treats each pixel from the event camera separately. The overall processing pipeline is shown in Algorithm \ref{pipelinealg}, and the IETS image generator is outlined in Algorithm \ref{stsalg}.

\begin{algorithm}
\caption{Inceptive Event Time Surfaces Processing Pipeline}
\label{pipelinealg}
\begin{algorithmic}[1]
\Procedure{Pipeline}{}\newline
\textbf{Input:} Event Files\newline
\textbf{Output:} Classification of Car or Background
\For{each data file}
  \State{Read in file events (100 ms of data)}
  \State{Process events into a Inceptive Event Time Surface}
\EndFor
\State{Execute Transfer Learning using Training Images}
\State{Evaluate Test Images through Classification Network}
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Inceptive Event Time Surfaces Algorithm}
\label{ietsalg}
\begin{algorithmic}[2]
\Procedure{Generate Inceptive Event Time Surface}{}\newline
\textbf{Input:} Events (points)\newline
\textbf{Output:} Inceptive Event Time Surface (MxNX3 Image)
\State{Initialize an MxNx3 zero array}
\For{each pixel with a negative event}
  \State{Calculate the IE}
  \If{IE exist}
    \State{Set red channel value for the pixel to IE time}
  \Else
    \State{Set red channel value for the pixel to average}
  \EndIf
\EndFor
\For{each pixel with an event}
  \State{Count the number of events at the pixel}
  \State{Set green channel value to the count}
\EndFor
\For{each pixel with a positive event}
  \State{Calculate the IE}
  \If{IE exist}
    \State{Set blue channel value for the pixel to IE time}
  \Else
    \State{Set blue channel value for the pixel to average}
  \EndIf
\EndFor
\State{Scale each channel from $0-1$}
\EndProcedure
\end{algorithmic}
\end{algorithm}
\fi


IETS produced overall better results than HATS. Some challenging cases for object classification are shown in Fig. \ref{fig:sts_miss_back} and Fig. \ref{fig:sts_miss_car}. Fig. \ref{fig:sts_miss_back} shows the STS image representation of background samples, and Fig. \ref{fig:sts_miss_car} shows the representation of car samples. Several of the datasets that were misclassified, were sparse in nature. Due to the nature of event cameras, if cars or background are collected with little to no relative camera motion, scenes generate few events independent of the scene. This will likely be a challenging collection of samples for any algorithm designed against the N-CARS dataset. Fig. \ref{fig:sts_correct_back} and Fig. \ref{fig:sts_correct_car} show successful classification from the STS algorithm. In each set of examples, there are cases that are challenging for classification by visual analysis. Some features that the algorithm is leveraging for classification appear to be car outlines, wheel motion, taillights, vertical poles/post, and signage. 
